CAZSL: Zero-Shot Regression for Pushing Models by Generalizing Through Context

Learning accurate models of the physical world is required for a lot of robotic manipulation tasks. However, during manipulation, robots are expected to interact with unknown workpieces so that building predictive models which can generalize over a number of these objects is highly desirable. In this paper, we study the problem of designing deep learning agents which can generalize their models of the physical world by building context-aware learning models. The purpose of these agents is to quickly adapt and/or generalize their notion of physics of interaction in the real world based on certain features about the interacting objects that provide different contexts to the predictive models. With this motivation, we present context-aware zero shot learning (CAZSL, pronounced as casual) models, an approach utilizing a Siamese network architecture, embedding space masking and regularization based on context variables which allows us to learn a model that can generalize to different parameters or features of the interacting objects. We test our proposed learning algorithm on the recently released Omnipush datatset that allows testing of meta-learning capabilities using low-dimensional data. Codes for CAZSL are available at https://www.merl.com/research/license/CAZSL.

==> tex/experiments_old.tex <==
\section{Experiments and Results}
We present results to clarify, motivate and justify the use of the proposed CAZSL method for zero-shot learning. To do so, we perform a series of numerical experiments to answer the following questions.
\begin{enumerate}
    \item Is the inclusion of context helpful towards learning?
    \item Does CAZSL improve regression performance on out-of-distribution samples?
    \item How should the distance function in CAZSL be selected?
\end{enumerate}

We evaluate our method on a simple regression task as well as six experiments using two contexts from the Omnipush dataset~\cite{bauza2019}. 
In the following subsections, we abbreviate competing methods evaluated as ANP (attentive neural process), FCN (fully-connected network), and FCN + CC (FCN with context concatenated to input). ANP~\cite{kim2019attentive} is a meta-learning method that uses an attention mechanism on relevant context points for regression, and FCN is a 4-layer fully-connected neural network. These two methods are used in the Omnipush data-release paper~\cite{bauza2019} and they do not make use of context information. 
We apply our proposed context mask and regularization directly on FCN for easy comparison of their effects.
We abbreviate variations of our proposed CAZSL method for ablation studies as FCN + CM (FCN with context mask), FCN + CM + L2Reg (FCN + CM with $L_2$ context regularization), and FCN + CM + NeuralReg (FCN + CM with neural context regularization).

We point out that the FCN predicts a Gaussian density for each sample as defined by a mean $\hat{y}_{t+1}$ and standard deviation $\hat{\sigma}$. The mean parameter is evaluated by root-mean-square error (RMSE). We also report the standard deviation (STD) to give a sense of the prediction uncertainty. All values reported correspond to test performance with parameters from the last training epoch. 

\textbf{Hyperparameters}: 
For the simple regression task in Section \ref{subsec:regression}, we train all models for $500$ epochs with the Adam optimizer using a learning rate of $\eta = 0.002$, and a batch size of $32$. This configuration is sufficient for convergence due to the small size of the simulation dataset.

For experiments on the Omnipush dataset in Section \ref{subsec:omnipush}, we use the same configurations as in \cite{bauza2019}, that is,
we train all models for a maximum of $3000$ epochs with the Adam optimizer using a learning rate $\eta = 0.002$, and a batch size of $64$. The ANP model in \cite{bauza2019} is trained for $5000$ epochs with warm-up step of $4000$ whereas we train for $3000$ epochs with warm-up step of $2000$ to match the number of epochs of all other methods. Our replicate results of methods in \cite{bauza2019} are comparable with the original results reported.

\subsection{Regression}
\label{subsec:regression}

We use a simple regression task to illustrate the effects of the proposed context mask and regularization on FCN.
We simulate 1D Gaussian processes with the RBF kernel:
\begin{equation*}
    K(a,b) = \xi^2 \exp\paren{-\frac{\|a-b\|^2}{2\ell}}
\end{equation*}
where $\xi$ controls the scale and $\ell$ is the bandwidth controlling how far the data can be extrapolated. The parameters are drawn uniformly at random as $\xi \sim \texttt {Unif}(0.1, 10)$ and $\ell \sim \texttt {Unif}(0.1, 10)$. The training set consists a total of 4000 samples extracted from Gaussian processes generated with 200 parameter sets. 20 samples are extracted per parameter set, and denoting $z_t$ as the observation at time $t$, each sample has predictor $x_t = \{z_{t-2}, z_{t-1}, z_t\}$ which is a subsequence of 3 historical observations and response $y_{t+1} = \{z_{t+1}\}$ as the predictive target. The context variable is the kernel parameters $c = \{\xi, \ell\}$. The test set consists 400 out-of-distribution samples corresponding to 20 new parameter sets.

The simulation is repeated 10 times. We set hyperparameters $\lambda_1 = 0.0001$ and $\lambda_2 = 10$ for the applicable models. We use a small degree of regularization since this regression task is relatively simple. 
From Table~\ref{tab: regression}, all variations of our proposed method outperform the baselines FCN and FCN + CC. 
We note that context concatenation has decreased accuracy while context masking has improved accuracy, which reflects the effectiveness of masking in the embedding space. 
The use of regularization further improves performance, and FCN + CM + L2Reg has the largest $9.26\%$ reduction of RMSE over FCN.

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
                                                                & RMSE           & STD            \\ \hline
FCN                                                             & 0.108          & 0.131          \\ \hline
\begin{tabular}[c]{@{}l@{}}FCN + CC\end{tabular}                & 0.146          & 0.133          \\ \hhline{|=|=|=|}
\begin{tabular}[c]{@{}l@{}}FCN + CM\end{tabular}                & 0.105          & 0.121          \\ \hline
\begin{tabular}[c]{@{}l@{}}FCN + CM + L2Reg\end{tabular}        & \textbf{0.098} & 0.100          \\ \hline
\begin{tabular}[c]{@{}l@{}}FCN + CM + NeuralReg\end{tabular}    & \underline{0.103}          &  0.113         \\ \hline
\end{tabular}
\caption{Average one-step prediction performance on out-of-distribution Gaussian processes samples across 10 simulations.\label{tab: regression}}
\end{table}

\subsection{Omnipush Dataset}
\label{subsec:omnipush}

\textbf{DataSet Description:}
The Omnipush dataset~\cite{bauza2019} collected 250 pushes per object for 250 objects on ABS surface (hard plastic). 
The data collection setup for pushing is shown in Figure~\ref{fig:exp_setup}. 
The objects are constructed to explore key factors that affect pushing -- the shape of the object and its mass distribution -- which have not been broadly explored in previous datasets and allow for study of generalization in model learning. 
Each side of the object has four possible shapes (concave, triangular, circular, rectangular) with three types of extra weights (0g, 60g, 150g). The triangular shape allows two positions (interior, exterior) for extra weights to be attached. A maximum of two weights are attached per object. We denote the shape and mass distribution of the objects as context, and experiment with two types of context variables:
\begin{enumerate}
    \item Indicator context: length--36 binary vector indicating the shape, extra weight and its position for each side
    \item Visual context: numerical array representing top-down view of object displayed in Figure~\ref{fig:data_sample}.
\end{enumerate}

This allows us to test the generalization capability of our proposed CAZSL technique. The visual context is $32\times 32$, resized from an original $481\times 481$ image\footnote{We resize original images in~\cite{bauza2019} using the resize function with default parameters in scikit-image.}. The dataset further has 250 pushes per object for 10 objects on plywood surface. 
More details of the dataset can be found on the website \url{http://web.mit.edu/mcube/omnipush-dataset/} and the corresponding paper~\cite{bauza2019}. 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.90\linewidth]{figure/setup_omnipush.png}
    %\vspace{-6pt}
	\caption{Omnipush dataset collection setup. The data is collected using an ABB industrial arm. The pusher is a steel rod attached to the end-effector of the arm. This steel arm interacts with the objects which are pushed during the experiments. The picture is reproduced with permission from~\cite{bauza2019}.}
	\label{fig:exp_setup}
\end{figure}

The prediction task is to estimate the ending location and orientation of the object after being pushed.
In data collection, the pusher is set to move at constant speed. Treating the location and angle of the object as the origin $\paren{x^{(o)}_t, y^{(o)}_t, a^{(o)}_t} = (0,0,0)$, the model input is $\paren{x^{(p)}_t, y^{(p)}_t, a^{(p)}_t}$ containing the location and angle of the pusher with respect to the object. The model output is the 3-dimensional vector $\paren{x^{(o)}_{t+1}, y^{(o)}_{t+1}, a^{(o)}_{t+1}}$.
To give a more intuitive representation of model accuracy, we convert RMSE to millimeters by multiplying it by 21.92mm, as done by the authors in \cite{bauza2019}.

\textbf{Experiment Setups:}
We use three setups to evaluate generalization performance of models across objects,
\begin{enumerate}
    \item \emph{Different objects}: training and test objects have different characteristics, that is, the combination of shapes, weights and weight positions for four sides;
    \item \emph{Different surfaces}: training objects are pushed on ABS surface and test objects are pushed on plywood;
    \item \emph{Different weights}: training and test objects have a different number of extra weights attached.
\end{enumerate}
The \emph{Different surfaces} setup allows evaluation for generalization performance beyond the provided context since surface information is not provided during training. We note that some objects pushed on plywood do not have images provided, and hence we only use indicator context for this setup. 

The \emph{Different weights} setup is further split into three sub-setups. There are three possible number of weights $\{0,1,2\}$ per object, and we use objects in each of the three options in turn as test objects, and the remaining objects as training objects.

For all experiments with indicator context, we set CAZSL hyperparameters $\lambda_1 = 0.01$ and $\lambda_2 = 10$ where applicable. For visual context, we set $\lambda = 0.01$ and $\lambda_2 = 0.01$ where applicable. The smaller $\lambda_2$ is to balance the higher dimensions of the visual context variables. When neural regularization is used, we treat $\lambda_2 = 1$ which is equivalent to not having the second hyperparameter.  

\textbf{Results:}
From Table~\ref{tab:diff_objnsurface} and \ref{tab:diff_wt}, CAZSL models consistently have improved performance over the baseline FCN and FCN + CC, reflecting that the inclusion of contextual information helps learning but the context should be applied to the embedding space instead of directly concatenated in the observation space. The RMSE of ANP is consistently between 0.22 and 0.28. Since ANP is a meta-learning method which is aimed at object-generalization, we would expect its performance to be fairly consistent across setups. In comparison with ANP, our CAZSL models achieved better performance except in 2 sub-cases in Table~\ref{tab:diff_wt_i} for learning \emph{Different weights} with indicator context. However, we note that our $L_2$ regularized approach outperforms the ANP in the $0$ weight test set of the \emph{Different weights} experiment, indicating the ability to better generalize to unknown mass distributions. Moreover, with the use of visual contexts which contain more detailed contextual information, CAZSL models consistently outperform ANP.

Comparing between the $L_2$ and neural regularizations in CAZSL models, we see that the former has lower RMSE when indicator context is used. Since the indicator context is a sparse binary vector, the neural network used for its embedding in neural regularization is possibly over-parameterized, hence resulting in overfitting. When visual context is used, the performance difference between the two choices of regularization is marginal. The convolutional neural network used for context embedding is able to extract spatial features possibly relating to the object geometry and mass distribution, and hence the kernel distance function learned is able to better discern differences between visual contexts. These results suggest that neural regularization is more suitable for complex or high-dimensional context variables. 

In summary, in all experiments, we find that our CAZSL models outperform baseline counterparts which do not implement context masking and regularization, and perform comparably or better than the ANP meta-learning baseline. We also observe that using indicator contexts improves performance over using no context most of the time, and using visual contexts improves performance over using indicator contexts or no context in all experiments. This suggests that increasing details in contextual information can be utilized to help learning.

\begin{table*}[h]
    \centering
    
    \begin{subtable}{\linewidth}
      \centering
      
        \begin{tabular}{| c | c | c | c | c | c | c |}
        \hline
        & \multicolumn{6}{c|}{Different objects} \\
        & \multicolumn{3}{c|}{Indicator context} & \multicolumn{3}{c|}{Visual context} \\ 
                            & RMSE          & STD       & Dist. (mm)        & RMSE      & STD       & Dist. (mm)       \\ \hline
        ANP                 & 0.228         & 0.080     & 5.00              & 0.228     & 0.080     & 5.00 \\ \hline
        FCN                 & 0.329         & 0.140     & 7.21              & 0.329     & 0.140 & 7.21\\ \hline
        FCN + CC            & 0.220         & 0.047     & 4.78              & 0.202     & 0.061     & 4.43 \\ \hhline{|=|=|=|=|=|=|=|}
        FCN + CM            & \underline{0.209}         & 0.029     & 4.58              & \underline{0.193}     & 0.041     & 4.23 \\ \hline
        FCN + CM + L2Reg    & \textbf{0.208}         & 0.031     & 4.56              & \textbf{0.192}     & 0.055     & 4.21 \\ \hline
        FCN + CM + NeuralReg& 0.220        &  0.035     & 4.78              & \underline{0.193}     & 0.067     & 4.23 \\ \hline
        \end{tabular}
        \caption{Different objects: Training and test samples are from objects with different characteristics i.e. shape and mass distribution.\label{tab:diff_obj}}
        
    \end{subtable}%    
    
    \begin{subtable}{\linewidth}
      \centering
      
        \begin{tabular}{| c | c | c | c |}
        \hline
        & \multicolumn{3}{c|}{Different surfaces: Indicator context} \\
                            &  RMSE     & STD       & Dist. (mm) \\ \hline
        ANP                 & 0.271     & 0.064     & 5.94          \\ \hline
        FCN                 & 0.333     & 0.146     & 7.30          \\ \hline
        FCN + CC            & 0.263     & 0.059     & 5.76          \\ \hhline{|=|=|=|=|}
        FCN + CM            & \textbf{0.255}     & 0.036     & 5.59          \\ \hline
        FCN + CM + L2Reg    & \textbf{0.255}     & 0.033     & 5.59          \\ \hline
        FCN + CM + NeuralReg& \underline{0.260}     & 0.045     & 5.70          \\ \hline
        \end{tabular}
        \caption{Different surfaces: Training samples are from objects pushed on ABS surface (hard plastic), and test samples are from objects pushed on plywood surface. Some test objects have different characteristics from training objects.\label{tab:diff_surface}}
        
    \end{subtable}%

    \caption{Method performance under multiple setups where test samples have out-of-distribution properties. Setups same as in \cite{bauza2019}. \label{tab:diff_objnsurface}}

\end{table*}
    
\begin{table*}[h]
    \centering
    \begin{subtable}{\linewidth}
      \centering
      
        \begin{tabular}{| c | c | c | c | c | c | c | c | c | c |}
        \hline
        & \multicolumn{9}{c|}{Different weights: Indicator context} \\
        & \multicolumn{3}{c|}{0 Weight} & \multicolumn{3}{c|}{1 Weight}  & \multicolumn{3}{c|}{2 Weights}\\
                            &  RMSE     & STD   & Dist. (mm)    &  RMSE     & STD   & Dist. (mm)    &  RMSE     & STD   & Dist. (mm) \\ \hline
        ANP                 &  0.264    & 0.079 & 5.79          &  \textbf{0.252}   & 0.066  & 5.52          &  \textbf{0.245}    & 0.080    & 5.37\\ \hline
        FCN                 &  0.330    & 0.144 & 7.23          &  0.356    & 0.125 & 7.80          &  0.326    & 0.157 & 7.15\\ \hline
        FCN + CC            &  0.261    & 0.047 & 5.72          &  0.390    & 0.035 & 8.55          &  0.320    & 0.064 & 7.01\\ \hhline{|=|=|=|=|=|=|=|=|=|=|}
        FCN + CM            &  \textbf{0.235}    & 0.033 & 5.15          &  0.267    & 0.030 & 5.85          &  \underline{0.269}    & 0.027 & 5.90\\ \hline
        FCN + CM + L2Reg    &  \underline{0.231}    & 0.038 & 5.06          &  \underline{0.256}    & 0.043 & 5.61          &  0.276    & 0.053 & 6.05\\ \hline
        FCN + CM + NeuralReg&  0.261    & 0.037 & 5.72          &  0.322    & 0.035 & 7.06          &  0.311    & 0.035 & 6.82\\ \hline
        \end{tabular}
        \caption{Different weights: Indicator context. \label{tab:diff_wt_i}}
        
    \end{subtable}%

    \begin{subtable}{\linewidth}
      \centering
      
        \begin{tabular}{| c | c | c | c | c | c | c | c | c | c |}
        \hline
        & \multicolumn{9}{c|}{Different weights: Visual context} \\
        & \multicolumn{3}{c|}{0 Weight} & \multicolumn{3}{c|}{1 Weight}  & \multicolumn{3}{c|}{2 Weights}\\
                            &  RMSE     & STD   & Dist. (mm)    &  RMSE     & STD   & Dist. (mm)    &  RMSE     & STD   & Dist. (mm) \\ \hline
        ANP                 &  0.264    & 0.079 & 5.79          &  0.252    & 0.066    & 5.52          &  0.245    & 0.080    & 5.37\\ \hline
        FCN                 &  0.330    & 0.144 & 7.23          &  0.356    & 0.125 & 7.80          &  0.326    & 0.157 & 7.15\\ \hline
        FCN + CC            &  0.235    & 0.040 & 5.15          & 0.282     & 0.045 & 6.18          & 0.269     & 0.065 & 5.90\\ \hhline{|=|=|=|=|=|=|=|=|=|=|}
        FCN + CM            &  0.223    & 0.033 & 4.89          & 0.231     & 0.034 & 5.06          & 0.222     & 0.040 & 4.87\\ \hline
        FCN + CM + L2Reg    &  \underline{0.210}    & 0.090 & 4.60          & \textbf{0.220}     & 0.051 & 4.82          & \textbf{0.218}     & 0.078 & 4.78\\ \hline
        FCN + CM + NeuralReg&  \textbf{0.208}    & 0.058 & 4.56          & \underline{0.222}     & 0.050 & 4.87          & \underline{0.220}     & 0.071 & 4.87\\ \hline
        \end{tabular}
        \caption{Different weights: Visual context.\label{tab:diff_wt_v}}
        
    \end{subtable}%
    
    \caption{Method performance when training and test samples are from objects with different number of weights attached, out of options from 0 to 2. For example, the heading `0 Weight' means that train samples are from objects with 1 or 2 weights attached, and test samples are from objects have no weight attached. Setup not in \cite{bauza2019}.\label{tab:diff_wt}}    

\end{table*}    
    
    
\iffalse
\begin{table*}{ht}
    \centering
    
    \begin{subtable}{\linewidth}
    \centering
    
        \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
        \hline
         & \multicolumn{6}{c|}{0 Weight} & \multicolumn{6}{c|}{1 Weight}  & \multicolumn{6}{c|}{2 Weights} \\
         & \multicolumn{3}{c|}{Indicator} & \multicolumn{3}{c|}{Visual} & \multicolumn{3}{c|}{Indicator} & \multicolumn{3}{c|}{Visual} & \multicolumn{3}{c|}{Indicator} & \multicolumn{3}{c|}{Visual} \\
                            & RMSE      & STD       & Dist. (mm) & RMSE      & STD       & Dist. (mm) & RMSE      & STD       & Dist. (mm)\\ \hline
        ANP                 & \\ \hline
        FCN                 & \\ \hline
        FCN + CC            & \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}
        FCN + CM            & \\ \hline
        FCN + CM + L2Reg    & \\ \hline
        FCN + CM + NeuralReg& \\ \hline
        \end{tabular}
        \caption{Different weights: Training and test samples are from objects with different number of weights attached, out of options from 0 to 2. For example, the heading `0 Weight' means that train samples are from objects with 1 or 2 weights attached, and test samples are from objects have no weight attached.}
    \end{subtable}
    
    \caption{Method performance under multiple setups where test samples have out-of-distribution properties.}
\end{table*}
\fi

